Improving Wikipedia Verifiability with AI

Verifiability is a core content policy of Wikipedia: claims that are likely to be challenged need to be backed by citations. There are millions of articles available online and thousands of new articles are released each month. For this reason, finding relevant sources is a difficult task: many claims do not have any references that support them. Furthermore, even existing citations might not support a given claim or become obsolete once the original source is updated or deleted. Hence, maintaining and improving the quality of Wikipedia references is an important challenge and there is a pressing need for better tools to assist humans in this effort. Here, we show that the process of improving references can be tackled with the help of artificial intelligence (AI). We develop a neural network based system, called Side, to identify Wikipedia citations that are unlikely to support their claims, and subsequently recommend better ones from the web. We train this model on existing Wikipedia references, therefore learning from the contributions and combined wisdom of thousands of Wikipedia editors. Using crowd-sourcing, we observe that for the top 10% most likely citations to be tagged as unverifiable by our system, humans prefer our system's suggested alternatives compared to the originally cited reference 70% of the time. To validate the applicability of our system, we built a demo to engage with the English-speaking Wikipedia community and find that Side's first citation recommendation collects over 60% more preferences than existing Wikipedia citations for the same top 10% most likely unverifiable claims according to Side. Our results indicate that an AI-based system could be used, in tandem with humans, to improve the verifiability of Wikipedia. More generally, we hope that our work can be used to assist fact checking efforts and increase the general trustworthiness of information online.

==> figures/RPcurve.tex <==
\if 0
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/RPcurve/RPcurve.pdf}
    \caption{Recall-Precision curve.}
    \label{fig:rpcurve}
\end{figure*}
\fi

\begin{figure*}[!t]
    \centering
    \begin{subfigure}[b]{0.43\textwidth}
        \includegraphics[width=\textwidth]{figures/RPcurve/RPcurve.pdf}
        \caption{Recall-Precision curve.}
    \label{fig:rpcurve}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.52\textwidth}
        \includegraphics[width=\textwidth]{figures/revisions.pdf}
        \caption{number of revisions vs failed verification score.}
        \label{fig:revisions}
    \end{subfigure}
    \caption{TBA.}
    \label{fig:rprevisions}
\end{figure*}

==> tables/bak_verifier_test.tex <==
\begin{table}[ht]
\centering
%\resizebox{\textwidth}{!}{
\begin{tabular}{lllllll}

 \toprule
  & \multicolumn{2}{c}{failed ver.} & \multicolumn{2}{c}{featured} & \multicolumn{2}{c}{random}  \\
 & True & False & True & False & True & False \\
 
 \midrule
 
 url depth > 1 & 72.01 & 27.99 & 92.68 & 7.32 & 93.42 & 6.58 \\
 url depth > 2 & 46.88 & 53.12 & 73.37 & 26.63 & 68.83 & 31.17 \\
 url depth > 3 & 29.62 & 70.38 & 52.6 & 47.4 & 47.21 & 52.79\\
 \midrule

BART & 60.73 & 39.27 & 81.09 & 18.91 & 75.14 & 24.86 \\
BART (url depth > 3) & 59.17 & 40.83 & 80.76 & 19.24 & 74.06 & 25.94\\


\bottomrule
\end{tabular}
%}
\caption{\label{tab:wafertest} Verifier test results.}
\end{table}

==> tables/expert_annotations.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{ll}
\hline
\toprule
No evidence & 41.3\% [52] \\
Partial evidence & 18.2\% [23] \\
Full evidence in one passage & 16.7\% [21] \\
Full evidence in multiple passages & 13.5\% [17] \\
Evidence in source but not in crawled text (e.g., multimedia) & 7.1\% [9] \\
Pay wall access & 3.2\% [4] \\
\bottomrule
\end{tabular}
\caption{Fine-grained human annotations for Wikipedia citations for which crowd annotators indicate no evidence. }
\label{tab:expert}
\end{table}

==> tables/legend.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{ll}
\hline
\toprule
split & data \\
\midrule
failed ver & 736\\
featured & 751\\
random & 3830\\
\bottomrule
\end{tabular}
\caption{\label{tab:example}Number of datapoints per split.}
\end{table}

==> tables/verifier_ranking.tex <==
\begin{table}[ht]
\centering
%\resizebox{\textwidth}{!}{
\begin{tabular}{lllllll}

 \toprule
   & \multicolumn{6}{c}{k} \\
 & 5 & 10 & 25 & 50 & 75 & 100 \\
 
 \midrule
 
BART & 100.0 & 90.0 & 48.0 & 46.0 & 38.67 & 33.0\\
BART (url depth > 3) & 40.0 & 40.0 & 24.0 & 18.0 & 26.67 & 24.0   \\

\bottomrule
\end{tabular}
%}
\caption{\label{tab:verifierranking} Verifier ranking test results vs k.}
\end{table}

==> tables/verifier_test.tex <==
\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llll}

 \toprule
  & \multicolumn{1}{c}{failed ver.} & \multicolumn{1}{c}{featured} & \multicolumn{1}{c}{random}  \\
 
 \midrule
 
 url depth > 1 &  27.99 & 92.68  & 93.42 \\
 url depth > 2 &  53.12 & 73.37  & 68.83  \\
 url depth > 3 &  70.38 & 52.6  & 47.21 \\
 \midrule

BART &  39.27 & 81.09  & 75.14  \\
BART (url depth > 3) & 40.83 & 80.76& 74.06 \\
BART constrained  & 41.17  & 80.16 & 75.07 \\
BART constrained (url depth > 3) & 42.66 & 79.24& - \\


\bottomrule
\end{tabular}
}
\caption{\label{tab:wafertest} Accuracy - Verifier test results.}
\end{table}

==> tables/wafer_dev.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lll}
\toprule
 &\multicolumn{2}{c}{micro avg.} \\
 & P@1 & SR@100 \\
\midrule
DPR pre-trained & 6.94 & 32.43 \\
BM25 & 18.42 & 60.05 \\
BM25 + Wikipedia title & 23.41 & 73.39 \\
GAR & \textbf{24.94} & 74.49 \\
GAR + Wikipedia title & 24.76 & \textbf{77.12} \\
\bottomrule
\end{tabular}
\caption{\label{tab:waferdev} WAFER dev results.}
\end{table}
